VM-Rec: A Variational Mapping Approach for Cold-start User Recommendation

The cold-start problem is a common challenge for most recommender systems. The practical application of most cold-start methods is hindered by the deficiency in auxiliary content information for users. Moreover, most methods necessitate simultaneous updates to the extensive parameters of recommender models, leading to significant training costs, particularly in large-scale industrial scenarios. We observe that the model can generate expressive embeddings for warm users with relatively more interactions. Initially, these users were cold-start users, and after transitioning to warm users, they exhibit clustering patterns in their embeddings with consistent initial interactions. Based on this motivation, we propose a Variational Mapping approach for cold-start user Recommendation (VM-Rec), mapping from few initial interactions to expressive embeddings for cold-start users. Specifically, we encode the initial interactions into a latent representation, where each dimension disentangledly signifies the degree of association with each warm user. Subsequently, we utilize this latent representation as the parameters for the mapping function, mapping (decoding) it into an expressive embedding, which can be integrated into a pre-trained recommender model directly. Our method is evaluated on three datasets using the same base model, demonstrating superior performance compared to other popular cold-start methods.

==> paper_252 <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{vib}
Alemi, A.A., Fischer, I., Dillon, J.V., Murphy, K.: Deep variational information bottleneck. arXiv preprint arXiv:1612.00410  (2016)

\bibitem{lastfm}
Cantador, I., Brusilovsky, P., Kuflik, T.: Second workshop on information heterogeneity and fusion in recommender systems (hetrec2011). In: Proceedings of the fifth ACM conference on Recommender systems. pp. 387--388 (2011)

\bibitem{chen2022generative}
Chen, H., Wang, Z., Huang, F., Huang, X., Xu, Y., Lin, Y., He, P., Li, Z.: Generative adversarial framework for cold-start item recommendation. In: Proceedings of the 45th International ACM SIGIR Conference on Research and Development in Information Retrieval. pp. 2565--2571 (2022)

\bibitem{dai2021poso}
Dai, S., Lin, H., Zhao, Z., Lin, J., Wu, H., Wang, Z., Yang, S., Liu, J.: Poso: Personalized cold start modules for large-scale recommender systems. arXiv preprint arXiv:2108.04690  (2021)

\bibitem{finn2017model}
Finn, C., Abbeel, P., Levine, S.: Model-agnostic meta-learning for fast adaptation of deep networks. In: International conference on machine learning. pp. 1126--1135. PMLR (2017)

\bibitem{gan}
Goodfellow, I., Pouget-Abadie, J., Mirza, M., Xu, B., Warde-Farley, D., Ozair, S., Courville, A., Bengio, Y.: Generative adversarial networks. Communications of the ACM  \textbf{63}(11),  139--144 (2020)

\bibitem{guo2016entity}
Guo, C., Berkhahn, F.: Entity embeddings of categorical variables. arXiv preprint arXiv:1604.06737  (2016)

\bibitem{hao2021pre}
Hao, B., Zhang, J., Yin, H., Li, C., Chen, H.: Pre-training graph neural networks for cold-start users and items representation. In: Proceedings of the 14th ACM International Conference on Web Search and Data Mining. pp. 265--273 (2021)

\bibitem{harper2015movielens}
Harper, F.M., Konstan, J.A.: The movielens datasets: History and context. Acm transactions on interactive intelligent systems (tiis)  \textbf{5}(4),  1--19 (2015)

\bibitem{lightgcn}
He, X., Deng, K., Wang, X., Li, Y., Zhang, Y., Wang, M.: Lightgcn: Simplifying and powering graph convolution network for recommendation. In: Proceedings of the 43rd International ACM SIGIR conference on research and development in Information Retrieval. pp. 639--648 (2020)

\bibitem{gumbel-softmax}
Jang, E., Gu, S., Poole, B.: Categorical reparameterization with gumbel-softmax. arXiv preprint arXiv:1611.01144  (2016)

\bibitem{kim2023meta}
Kim, M., Yang, Y., Ryu, J.H., Kim, T.: Meta-learning with adaptive weighted loss for imbalanced cold-start recommendation. arXiv preprint arXiv:2302.14640  (2023)

\bibitem{kingma2013auto}
Kingma, D.P., Welling, M.: Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114  (2013)

\bibitem{lee2019melu}
Lee, H., Im, J., Jang, S., Cho, H., Chung, S.: Melu: Meta-learned user preference estimator for cold-start recommendation. In: Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining. pp. 1073--1082 (2019)

\bibitem{liu2023Boosting}
Liu, H., Lin, H., Zhang, X., Ma, F., Chen, H., Wang, L., Yu, H., Zhang, X.: Boosting meta-learning cold-start recommendation with graph neural network. In: Proceedings of the 32nd ACM International Conference on Information and Knowledge Management. p. 4105–4109. CIKM '23 (2023)

\bibitem{lu2020meta}
Lu, Y., Fang, Y., Shi, C.: Meta-learning on heterogeneous information networks for cold-start recommendation. In: Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining. pp. 1563--1573 (2020)

\bibitem{van2008visualizing}
Van~der Maaten, L., Hinton, G.: Visualizing data using t-sne. Journal of machine learning research  \textbf{9}(11) (2008)

\bibitem{sas}
Mitchell, T.J., Beauchamp, J.J.: Bayesian variable selection in linear regression. Journal of the american statistical association  \textbf{83}(404),  1023--1032 (1988)

\bibitem{ouyang2021learning}
Ouyang, W., Zhang, X., Ren, S., Li, L., Zhang, K., Luo, J., Liu, Z., Du, Y.: Learning graph meta embeddings for cold-start ads in click-through rate prediction. In: Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval. pp. 1157--1166 (2021)

\bibitem{metaemb}
Pan, F., Li, S., Ao, X., Tang, P., He, Q.: Warm up cold-start advertisements: Improving ctr predictions via learning to learn id embeddings. In: Proceedings of the 42nd International ACM SIGIR Conference on Research and Development in Information Retrieval. pp. 695--704 (2019)

\bibitem{bpr}
Rendle, S., Freudenthaler, C., Gantner, Z., Schmidt-Thieme, L.: Bpr: Bayesian personalized ranking from implicit feedback. arXiv preprint arXiv:1205.2618  (2012)

\bibitem{taobao}
Tianchi: Ad display/click data on taobao.com (2018), \url{https://tianchi.aliyun.com/dataset/dataDetail?dataId=56}

\bibitem{tishby2000information}
Tishby, N., Pereira, F.C., Bialek, W.: The information bottleneck method. arXiv preprint physics/0004057  (2000)

\bibitem{titsias2011spike}
Titsias, M., L{\'a}zaro-Gredilla, M.: Spike and slab variational inference for multi-task and multiple kernel learning. Advances in neural information processing systems  \textbf{24} (2011)

\bibitem{vaswani2017attention}
Vaswani, A., Shazeer, N., Parmar, N., Uszkoreit, J., Jones, L., Gomez, A.N., Kaiser, {\L}., Polosukhin, I.: Attention is all you need. Advances in neural information processing systems  \textbf{30} (2017)

\bibitem{dropoutnet}
Volkovs, M., Yu, G., Poutanen, T.: Dropoutnet: Addressing cold start in recommender systems. Advances in neural information processing systems  \textbf{30} (2017)

\bibitem{neuralgcf}
Wang, X., He, X., Wang, M., Feng, F., Chua, T.S.: Neural graph collaborative filtering. In: Proceedings of the 42nd international ACM SIGIR conference on Research and development in Information Retrieval. pp. 165--174 (2019)

\bibitem{metacf}
Wei, T., Wu, Z., Li, R., Hu, Z., Feng, F., He, X., Sun, Y., Wang, W.: Fast adaptation for cold-start collaborative filtering with meta-learning. In: 2020 IEEE International Conference on Data Mining (ICDM). pp. 661--670. IEEE (2020)

\bibitem{wei2021contrastive}
Wei, Y., Wang, X., Li, Q., Nie, L., Li, Y., Li, X., Chua, T.S.: Contrastive learning for cold-start recommendation. In: Proceedings of the 29th ACM International Conference on Multimedia. pp. 5382--5390 (2021)

\bibitem{wdof}
Wen, J., Liu, H., Jing, L.: Modeling preference as weighted distribution over functions for user cold-start recommendation. In: Proceedings of the 32nd ACM International Conference on Information and Knowledge Management. p. 2706–2715. CIKM '23 (2023)

\bibitem{recbole[1.1.1]}
Xu, L., Tian, Z., Zhang, G., Wang, L., Zhang, J., Zheng, B., Li, Y., Hou, Y., Pan, X., Chen, Y., Zhao, W.X., Chen, X., Wen, J.R.: Recent advances in recbole: Extensions with more practical considerations (2022)

\bibitem{velf}
Xu, X., Yang, C., Yu, Q., Fang, Z., Wang, J., Fan, C., He, Y., Peng, C., Lin, Z., Shao, J.: Alleviating cold-start problem in ctr prediction with a variational embedding learning framework. In: Proceedings of the ACM Web Conference 2022. pp. 27--35 (2022)

\bibitem{yuan2020parameter}
Yuan, F., He, X., Karatzoglou, A., Zhang, L.: Parameter-efficient transfer from sequential behaviors for user modeling and recommendation. In: Proceedings of the 43rd International ACM SIGIR conference on research and development in Information Retrieval. pp. 1469--1478 (2020)

\bibitem{yuan2023go}
Yuan, Z., Yuan, F., Song, Y., Li, Y., Fu, J., Yang, F., Pan, Y., Ni, Y.: Where to go next for recommender systems? id-vs. modality-based recommender models revisited. arXiv preprint arXiv:2303.13835  (2023)

\bibitem{zhao2018learning}
Zhao, K., Li, Y., Shuai, Z., Yang, C.: Learning and transferring ids representation in e-commerce. In: Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining. pp. 1031--1039 (2018)

\bibitem{zhao2022improving}
Zhao, X., Ren, Y., Du, Y., Zhang, S., Wang, N.: Improving item cold-start recommendation via model-agnostic conditional variational autoencoder. In: Proceedings of the 45th International ACM SIGIR Conference on Research and Development in Information Retrieval. pp. 2595--2600 (2022)

\bibitem{zhou2023contrastive}
Zhou, Z., Zhang, L., Yang, N.: Contrastive collaborative filtering for cold-start item recommendation. arXiv preprint arXiv:2302.02151  (2023)

\bibitem{mwuf}
Zhu, Y., Xie, R., Zhuang, F., Ge, K., Sun, Y., Zhang, X., Lin, L., Cao, J.: Learning to warm up cold item embeddings for cold-start recommendation with meta scaling and shifting networks. In: Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval. pp. 1167--1176 (2021)

\bibitem{zhu2020recommendation}
Zhu, Z., Sefati, S., Saadatpanah, P., Caverlee, J.: Recommendation for new users and new items via randomized training and mixture-of-experts transformation. In: Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval. pp. 1121--1130 (2020)

\end{thebibliography}

